HD-Eval: Aligning Large Language Model Evaluators Through Hierarchical Criteria Decomposition

Large language models (LLMs) have emerged as a promising alternative to expensive human evaluations. However, the alignment and coverage of LLM-based evaluations are often limited by the scope and potential bias of the evaluation prompts and criteria. To address this challenge, we propose HD-Eval, a novel framework that iteratively aligns LLM-based evaluators with human preference via Hierarchical Criteria Decomposition. HD-Eval inherits the essence from the evaluation mindset of human experts and enhances the alignment of LLM-based evaluators by decomposing a given evaluation task into finer-grained criteria, aggregating them according to estimated human preferences, pruning insignificant criteria with attribution, and further decomposing significant criteria. By integrating these steps within an iterative alignment training process, we obtain a hierarchical decomposition of criteria that comprehensively captures aspects of natural language at multiple levels of granularity. Implemented as a white box, the human preference-guided aggregator is efficient to train and more explainable than relying solely on prompting, and its independence from model parameters makes it applicable to closed-source LLMs. Extensive experiments on three evaluation domains demonstrate the superiority of HD-Eval in further aligning state-of-the-art evaluators and providing deeper insights into the explanation of evaluation results and the task itself.

==> Figures/decomp_prompt.tex <==
\begin{figure*}[!t]
\centering
\begin{tcolorbox}[width=1\textwidth, fontupper=\small, colback=blue!2, boxrule=0.9pt] 
\#\# Instructions

Score the following summary of a news article on its \textcolor{purple}{[Aspect]}.

Please return your score on how the summary is \textcolor{purple}{[Aspect]} with the article in the scale of 1 to 5, with 1 being the lowest.\\

\#\# Example

\textcolor{blue}{[Article and Summary to be evaluated]} \\

\#\# Criteria for \textcolor{purple}{[Aspect]}

\textcolor{blue}{[Calibrated criteria for evaluating this aspect]} \\

\#\# Evaluation

Now, please evaluate how \textcolor{purple}{[Aspect]} is the summary to the article (on a scale of 1-5, with 1 being the lowest).
Please carefully read the article and summary, and follow the scoring criteria above to score the \textcolor{purple}{[Aspect]} of the summary to the article.

Please first return your score, and then provide your reasoning for the score. \\

\textcolor{purple}{[Aspect]} Score (1-5):
\end{tcolorbox}
\caption{Prompt template for evaluation on text summarization (SummEval, NewsRoom).}
\label{fig:eval-summ}
\end{figure*}

\begin{figure*}[!t]
\centering
\begin{tcolorbox}[width=1\textwidth, fontupper=\small, colback=blue!2, boxrule=0.9pt] 
\#\# Instructions

Please score on the \textcolor{purple}{[Aspect]} of a following natural language sentence generated according to a structured data expression.

Please return your score on how \textcolor{purple}{[Aspect]} is the sentence, in the scale of 1 to 6, with 1 being the lowest. \\


\#\# Example

\textcolor{blue}{[Data expression and text to be evaluated]} \\

\#\# Criteria for \textcolor{purple}{[Aspect]}

\textcolor{blue}{[Calibrated criteria for evaluating this aspect]} \\

\#\# Evaluation

Now, please evaluate how \textcolor{purple}{[Aspect]} is the generated sentence. (on a scale of 1-6, with 1 being the lowest)
Please carefully read the sentence and the structured data expression, and follow the scoring criteria to score the \textcolor{purple}{[Aspect]} of the sentence.

Please first return your score, and then provide your reasoning for the score. \\

\textcolor{purple}{[Aspect]} Score (1-5):
\end{tcolorbox}
\caption{Prompt template for evaluation on data-to-text (SFRES, SFHOT).}
\label{fig:eval-d2t}
\end{figure*}


\begin{figure*}[!t]
\centering
\begin{tcolorbox}[width=1\textwidth, fontupper=\small, colback=blue!2, boxrule=0.9pt] Is the sentence supported by the article?

Answer 1 if the summary is factually consistent with the article, 0 otherwise.\\

\textcolor{blue}{[Article and Summary to be evaluated]} \\

\textcolor{blue}{[Calibrated criteria for evaluating hallucination]} \\

Answer:
\end{tcolorbox}
\caption{Prompt template for evaluation on evaluating hallucinations (QAGS-XSUM/CNN).}
\label{fig:eval-qags}
\end{figure*}


==> Tables/case_decmp.tex <==
\begin{table*}[t]
\centering
\footnotesize
\resizebox{0.98\textwidth}{!}{
\begin{tabular}{p{0.96\textwidth}}
\toprule
\textbf{Criteria Decomposition} - Dialogue Generation \\ \midrule
\cellcolor[rgb]{ .915,  .915,  .915} \textit{\textbf{Layer 1} Decomposition} \\
$\clubsuit:$ Naturalness (\textcolor{violet}{\textit{nat}}), $\diamondsuit:$ Coherence (\textcolor{violet}{\textit{coh}}), $\spadesuit:$ Engagingness (\textcolor{violet}{\textit{eng}}), $\heartsuit:$ Groundedness (\textcolor{violet}{\textit{grd}}) \\

\cellcolor[rgb]{ .915,  .915,  .915} \textit{\textbf{Layer 2} Decomposition} \\
$\clubsuit:$ Grammar and syntax (\textcolor{violet}{\textit{gram}}), \underline{Spelling and punctuation} (\textcolor{violet}{\textit{spell}}), Lexical choice and diversity (\textcolor{violet}{\textit{div}})\\

$\diamondsuit:$ Topic relevance (\textcolor{violet}{\textit{topic}}), Logical flow (\textcolor{violet}{\textit{logic}}), Context consistency (\textcolor{violet}{\textit{context}})\\

$\spadesuit:$ \underline{Content richness} (\textcolor{violet}{\textit{contr}}), Emotional engagement (\textcolor{violet}{\textit{emo}}), \underline{Feedback} (\textcolor{violet}{\textit{feedback}}), User involvement (\textcolor{violet}{\textit{userinv}})\\

$\heartsuit:$ Factual consistency (\textcolor{violet}{\textit{factcon}}), \underline{Factual accuracy} (\textcolor{violet}{\textit{factacc}}), Knowledge (\textcolor{violet}{\textit{knowle}}), Consistency (\textcolor{violet}{\textit{con}}) \\

\cellcolor[rgb]{ .915,  .915,  .915} \textit{\textbf{Layer 3} Decomposition} \\

\underline{$\clubsuit:$} Spelling correctness (\textcolor{violet}{\textit{spcorr}}), Punctuation correctness (\textcolor{violet}{\textit{puncorr}})\\

\underline{$\spadesuit:$} Information quantity (\textcolor{violet}{\textit{infoquant}}), Information quality (\textcolor{violet}{\textit{infoqual}}), Topic diversity (\textcolor{violet}{\textit{topdiv}}), Topic relevance (\textcolor{violet}{\textit{toprel}}); \\
\quad\ \, Length (\textcolor{violet}{\textit{length}}), Tone (\textcolor{violet}{\textit{tone}}), Engagement (\textcolor{violet}{\textit{engage}}) \\

\underline{$\heartsuit:$} Factual correctness (\textcolor{violet}{\textit{factcorr}}), Factual source (\textcolor{violet}{\textit{factsource}}), Factual relevance (\textcolor{violet}{\textit{factrel}})\\


\bottomrule
\end{tabular}}
\caption{A case study for criteria decomposition on Topical-Chat. \underline{Underlined} denote criteria being selected with attribution pruning. Note that we also generate a \textit{description} of criteria in parallel, which is omitted due to space.}
\label{tab:case}
\end{table*}
